GeRM: A Generative Rendering Model From Physically Realistic to Photorealistic

While physically-based rendering (PBR) simulates light transport that guarantees physical realism, achieving true photorealistic rendering (PRR) demands prohibitive time and labor, and still struggles to capture the intractable richness of the real world. We propose GeRM, the first multimodal generative rendering model to bridge the gap from PBR to PRR (P2P). We formulate this P2P transition by learning a distribution transfer vector (DTV) field to direct the generative process. To achieve this, we introduce a multi-condition ControlNet that synthesizes PBR images and progressively transitions them into PRR images, guided by G-buffers, text prompts, and cues for enhanced regions. To improve the model's grasp of the image distribution shift driven by text prompts, we propose a residual perceptual transfer mechanism to associate text prompts with corresponding targeted modification regions, which more clearly defines the incremental component updates. To supervise this transfer process, we introduce a multi-agent visual language model framework to construct an expert-guided pairwise transfer dataset, named P2P-50K, where each paired sample corresponds to a specific transfer vector in the DTV field. Extensive experiments demonstrate that GeRM synthesizes high-quality controllable images and outperforms state-of-the-art baselines across diverse applications, including PBR and PRR image synthesis and editing.

==> section/3_preliminary.tex <==
\section{Preliminary}
\label{sec:preliminary}
% \subsection{Diffusion Model}
% Diffusion models operate through a two-phase process: a forward and a backward process. In the forward process, starting from an initial data point \( x_0 \) sampled from the true data distribution, Gaussian noise is incrementally added to create a series of intermediate states \( x_1, x_2, \ldots, x_T \), with \( x_T \) approaching a standard Gaussian distribution. In latent diffusion models~\citep{rombach2022high}, the diffusion process is conducted in the latent space via a pre-trained variational autoencoder (VAE), which can be mathematically represented as 
% \begin{equation}
% z_t = \sqrt{\overline\alpha_t} z_0 + \sqrt{1 - \overline\alpha_t} \epsilon,  where \; \epsilon \sim \mathcal{N}(0, I), \label{1}
% \end{equation}
% where \( z_t \) is the noisy latent feature at time step \( t \), \( z_0 \) is the initial data in latent space, \( \epsilon \) is the Gaussian noise, and \( \overline\alpha_t \) is the parameter of noise strength at time step \( t \). Conversely, the backward process involves starting from a noisy data point \( x_T \) sampled from the standard Gaussian distribution and progressively removing the noise to generate intermediate states \( x_{T-1}, x_{T-2}, \ldots, x_0 \). During this denoising process, a U-Net \( \epsilon_\theta(\cdot) \) ~\citep{ronneberger2015u} is learnt to predict the noise at time step \( t \), with the MSE loss
% \begin{equation}
% \mathcal{L} = \mathbb{E}_{z_0, \epsilon, t}[\left \| \epsilon - \epsilon_\theta(z_t, t)\right \|_2^2].
% \end{equation}
% For text-to-image diffusion models~\citep{ramesh2022hierarchical}, the text prompt is used to guide the generation process. A text prompt \( y \) is converted into a sequence of vectors using a text encoder \( \tau_\theta(\cdot) \) and mixed with the attention layers of the U-Net. The training process can be optimized via
% \begin{equation}
% \mathcal{L} = \mathbb{E}_{z_0, y, \epsilon, t}[\left \| \epsilon - \epsilon_\theta(z_t, t, \tau_\theta(y))\right \|_2^2].
% \end{equation}
% To accommodate more complex control conditions, ControlNet~\citep{zhang2023adding} introduces a control branch that leverages image information as a conditioning factor to guide the generation process. This innovation enables precise control over image generation, resulting in high-quality outputs. The generative diffusion model can be trained with the loss
% \begin{equation}
% \mathcal{L} = \mathbb{E}_{z_0, y, \epsilon, t, c_I}[\left \| \epsilon - \epsilon_\theta(z_t, t, \tau_\theta(y), c_I)\right \|_2^2], \label{4}
% \end{equation}
% where \( c_I \) is the encoded conditional image.
\subsection{Traditional Graphics Pipeline}
Traditional graphics engines have long been dedicated to solving similar problems:
\begin{equation}
I = R(a,r,m,n,d,o,l),
\label{eq:engine_problem}
\end{equation}
where \(I\) denotes the generated images, $R$ represents the rendering layer, and $a, r, m, n, d$ corresponds to albedo, roughness, metallic, normal, and depth within the current viewport. $o$ represents the geometric information of the entire scene outside the viewport, and $l$ corresponds to the lighting in the scene. 


==> section/7_figures.tex <==






% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=1\linewidth]{figures/pdf/sig_ablation.pdf}
%     \vspace{-0.3cm}
%     \caption{Qualitative results of the ablation study. Further discussion can be found in~\refSec{sec:ablation}.}
%     \label{fig:ablation}
%     \vspace{-0.3cm}
% \end{figure*}

==> section/paper_list.tex <==
\section{Paper List (Temp Section)}
\wzz{work on listing paper now}
\subsection{Temporal Reconstruction for Real-time Rendering}
\cc{
General:
\begin{enumerate}
    \item Temporal Coherence Methods in Real-Time Rendering \cite{scherzer2012temporal}
\end{enumerate}
non-Neural, Temoral, Spatiotemporal: 
\begin{enumerate}
    \item Spatiotemporal variance-guided filtering: real-time reconstruction for path-traced global illumination \cite{schied2017spatiotemporal} 
\end{enumerate}
Neural, Temoral, non-image:
\begin{enumerate}
    \item Real-time Neural Radiance Caching for Path Tracing \cite{muller2021real}
\end{enumerate}
Neural, frame-rate up:
\begin{enumerate}
    \item Nerual Frame Interpolation for Rendered Content \cite{briedis2021neural} 
    \item ExtraNet: real-time extrapolated rendering for low-latency temporal supersampling \cite{guo2021extranet}
\end{enumerate}
Neural, Denoising / AA:
\begin{enumerate}
    \item A reduced-precision network for image reconstruction \cite{thomas2020reduced}
    \item Neural temporal adaptive sampling and denoising \cite{hasselgren2020neural}
    \item Interactive Monte Carlo Denoising using Affinity of Neural Features \cite{icsik2021interactive}
\end{enumerate}
Neural, supersampling:
\begin{enumerate}
    \item Neural supersampling for real-time rendering \cite{xiao2020neural}
    \item Classifier Guided Temporal Supersampling for Real-time Rendering \cite{guo2022classifier}
    \item Temporally Stable Real-Time Joint Neural Denoising and Supersampling \cite{thomas2022temporally}
\end{enumerate}
we use both temporal and spatial warping when encoding feature.
}
\subsection{Deep Video Frame Interpolation}
\cc{
Flow-based: 
\begin{enumerate}
    \item Video Frame Synthesis using Deep Voxel Flow
    \item Super slomo: High quality estimation of multiple intermediate frames for video interpolation \cite{jiang2018super}
    \item Depth-aware video frame interpolation \cite{bao2019depth}
    \item Quadratic video interpolation \cite{xu2019quadratic}
    \item Enhanced quadratic video interpolation \cite{liu2020enhanced}
    \item Video enhancement with task-oriented flow.
    \item Adaptive Collaboration of Flows for Video Frame Interpolation
    \item Softmax splatting for video frame interpolation \cite{niklaus2020softmax}
    \item BMBC: Bilateral motion estimation with bilateral cost volume for video interpolation \cite{park2020bmbc}
    \item A flexible recurrent residual pyramid network for video frame intefrpolation.
    \item Asymmetric Bilateral Motion Estimation for Video Frame Interpolation \cite{park2021asymmetric}
    \item Rife: Real-time intermediate flow estimation for video frame interpolation \cite{huang2022real}
    \item IFRNet: Intermediate Feature Refine Network for Efficient Frame Interpolation\cite{kong2022ifrnet} 
    \item Long-Term Video Frame Interpolation via Feature Propagation \cite{Argaw_2022_CVPR}
\end{enumerate}
Kernel-based:
\begin{enumerate}
        \item Video frame interpolation via adaptive separable convolution \cite{niklaus2017video}
        \item Channel Attention Is All You Need for Video Frame Interpolation \cite{choi2020channel}
        \item Video frame interpolation via deformable separable convolution \cite{cheng2020video}
        \item Flow-Agnostic Video Representations for Fast Frame Interpolation \cite{kalluri2020flavr}
        \item Multiple video frame interpolation via enhanced deformable separable convolution \cite{cheng2021multiple}
\end{enumerate}
Kernel and Flow Combined:
\begin{enumerate}
    \item Memc-net: Motion estimation and motion compensation driven neural network for video interpolation and enhancement \cite{bao2019memc}
\end{enumerate}
Phase-based: \\
Hallucination-based (Image Generation): \\
Others:
\begin{enumerate}
    \item AdaCoF: Adaptive Collaboration of Flows for Video Frame Interpolation \cite{lee2020adacof}
    \item Compression-Driven Network Design for Frame Interpolation \cite{ding2021cdfi}
    \item Many-to-many Splatting for Efficient Video Frame Interpolation \cite{hu2022many}
\end{enumerate}
Animation:
\begin{enumerate}
    \item Deep animation video interpolation in the wild \cite{siyao2021deep}
    \item Enhanced Deep Animation Video Interpolation \cite{shen2022enhanced}
    \item Deep Animation Video Interpolation in the Wild
    \item Improving the Perceptual Quality of 2D Animation Interpolation
\end{enumerate}
}
\subsection{Flow Estimation and Motion Compensation}
\cc{
Supervised:
\begin{enumerate}
    \item An iterative image registration technique with an application to stereo vision
    \item Estimating optical flow by integrating multi-frame information
    \item FlowNet: Learning Optical Flow With Convolutional Networks \cite{Dosovitskiy_2015_ICCV}: FlowNet\cite{Dosovitskiy_2015_ICCV} firsly shows convolutional neural networks can predict per-pixel optical flow filed with artificially generated datasets, but it suffers from noisy and blurry result.
    \item FlowNet 2.0: Evolution of Optical Flow Estimation with Deep Networks \cite{2017FlowNet}: FlowNet2.0\cite{2017FlowNet} stacks FlowNets to get more robust optical flow by a coarse-to-fine training process, and use network with smaller stride and kernel size to handle small displacement case.
    \item Optical flow estimation using a spatial pyramid network \cite{ranjan2017optical}: Ranjan et al. \shortcite{ranjan2017optical} introduce SpyNet based on spatial pyramid method to learn residual flow in a multi-scale sequence. SpyNet uses much smaller network since slight motion between the first and the warped second images easier to estimate in every scale, but it has bad quality in scenes including large motion.
    \item Pwc-net: Cnns for optical flow using pyramid, warping, and cost volume \cite{sun2018pwc}: PWC-Net \cite{sun2018pwc} extends image warping to feature warping also in a pyramid structure, and uses warped feature to compute cost volume, which improves the result still with lightweight network.
    \item Liteflownet: A lightweight convolutional neural network for optical flow estimation \cite{hui2018liteflownet}: Hui et al. \shortcite{hui2018liteflownet} introduces LiteFlowNet which leverage pyramid feature warping to predict optiacal flow by cascaded flow inference and flow regularization.
    \item Iterative Residual Refinement for Joint Optical Flow and Occlusion Estimation \cite{hur2019iterative}: Hur et al.\shortcite{hur2019iterative} proposed an iterative residual refinement method, which can increase the accuracy of existing networks by just adopting this IRR scheme to each iteration of FlowNet or each pyramid level of PWC-Net without inflation of parameters.
    \item Hierarchical discrete distribution decomposition for match density estimation \cite{yin2019hierarchical}
    \item LiteFlowNet2, A Lightweight Optical Flow CNN —Revisiting Data Fidelity and Regularization \cite{hui2020lightweight}: faster and more accurate LiteFlowNet2.
    \item Liteflownet3: Resolving correspondence ambiguity for more accurate optical flow estimation \cite{hui2020liteflownet3}: Hui et al. \shortcite{hui2020liteflownet3} improves LiteFlowNet by removing outliers in cost volume and deforming inaccurate values in flow field.
    \item RAFT:  Recurrent all-pairs field transforms for optical flow \cite{teed2020raft}: Unlike mainstream pyramid-based method, RAFT \cite{teed2020raft} builds multi-scale pixel-wise 4D correlation volumes according to the visual similarity, and preforms a recurrent update operator to calculate feature map and refine the flow iteratively.
    \item A Lightweight Network Model For Video Frame Interpolation Using Spatial Pyramids \cite{zhuang2020lightweight}
    \item ScopeFlow: Dynamic Scene Scoping for Optical Flow \cite{Bar_Haim_2020_CVPR}: crop inputs for new training scheme.
    \item STaRFlow: A spatiotemporal recurrent cell for lightweight multi-frame optical flow estimation \cite{godet2021starflow}:  STaRFlow\shortcite{godet2021starflow} is a lightweight model with spatiotemporal recurrence for multi-frame for jointly estimating optical flow and occlusion.
    \item Learning to Estimate Hidden Motions with Global Motion Aggregation \cite{jiang2021learning}: \cite{jiang2021learning} uses attention mechanism of Transformer to resolve motion of occluded pixel by a global motion feature aggregation, which lifts drawback of limited range of CNNs.
    \item High-resolution optical flow from 1d attention and correlation \cite{xu2021high}
    \item GMFlow: Learning Optical Flow via Global Matching \cite{xu2022gmflow}: GMFlow solves optical flow as a global matching problem with a Transformer for feature enhancement.
    \item FlowFormer: A Transformer Architecture for Optical Flow \cite{huang2022flowformer}: FlowFormer \cite{huang2022flowformer} integrates a Image-Net-pretrained Transformer into a new encoder-decoder structure, which can aggregate cost volume into impact latent cost tokens.
    \item NVIDIA Optical Flow SDK
\end{enumerate}
Unsupervised: 
\begin{enumerate}
    \item DenseNet for dense flow \cite{zhu2017densenet}
    \item Unsupervised deep learning for optical flow estimation \cite{ren2017unsupervised}
    \item Unsupervised learning of multi-frame optical flow with occlusions \cite{janai2018unsupervised}
    \item Unflow: Unsupervised learning of optical flow with a bidirectional census loss \cite{meister2018unflow}: Inspired by energy-based flow approaches, UnFlow \cite{meister2018unflow} defines occlusion constraint, occlusion-aware data loss based on census transform and higher-order smoothness.
    \item DDFlow: Learning Optical Flow with Unlabeled Data Distillation \cite{liu2019ddflow}: Liu et al. \shortcite{liu2019ddflow} presents a teacher-student data distillation approach.
    \item SelFlow: Self-Supervised Learning of Optical Flow \cite{liu2019selflow}: Liu et al. \shortcite{liu2019selflow} trains neural network on non-occlusion multi-frame input, and then fine-tunes on images injected with random noise into superpixels.
    \item What Matters in Unsupervised Optical Flow
    \item Learning by Analogy: Reliable Supervision from Transformations for Unsupervised Optical Flow Estimation \cite{liu2020learning}
    \item Separable Flow: Learning Motion Cost Volumes for Optical Flow Estimation \cite{Zhang_2021_ICCV}
    \item Feature-Level Collaboration: Joint Unsupervised Learning of Optical Flow, Stereo Depth and Camera Motion \cite{Chi_2021_CVPR}
    \item OccInpFlow: Occlusion-Inpainting Optical Flow Estimation by Unsupervised Learning
    \item UPFlow: Upsampling Pyramid for Unsupervised Optical Flow Learning
    \item Optical Flow Training under Limited Label Budget via Active Learning
\end{enumerate}
CG: 
\begin{enumerate}
    \item Temporally Reliable Motion Vectors for Real-time Ray Tracing \cite{zeng2021temporally}
\end{enumerate}
\subsection{Video Prediction}
\cc{
RNN: 
\begin{enumerate}
    \item Video (language) modeling: a baseline for generative models of natural videos \cite{ranzato2014video}
    \item Predrnn: Recurrent neural networks for predictive learning using spatiotemporal lstms \cite{wang2017predrnn}
    \item Predrnn++: Towards a resolution of the deep-in-time dilemma in spatiotemporal predictive learning \cite{wang2018predrnn++}
    \item Eidetic 3D LSTM: A model for video prediction and beyond \cite{wang2018eidetic}
    \item Predrnn: A recurrent neural network for spatiotemporal predictive learning \cite{wang2022predrnn}
\end{enumerate}
autoencoder:
\begin{enumerate}
        \item FitVid: Overfitting in pixel-level video prediction \cite{babaeizadeh2021fitvid}
        \item Clockwork variational autoencoders \cite{saxena2021clockwork}
\end{enumerate}
GAN:
\begin{enumerate}
    \item Adversarial video generation on complex datasets \cite{clark2019adversarial}
    \item Transformation-based adversarial video prediction on large-scale data \cite{luc2020transformation}
\end{enumerate}
diffusion model:
\begin{enumerate}
    \item Diffusion models for video prediction and infilling \cite{hoppe2022diffusion}
\end{enumerate}
}
}
